A Survey of Reinforcement Learning For Economics

This survey (re)introduces reinforcement learning methods to economists. The curse of dimensionality limits how far exact dynamic programming can be effectively applied, forcing us to rely on suitably "small" problems or our ability to convert "big" problems into smaller ones. While this reduction has been sufficient for many classical applications, a growing class of economic models resists such reduction. Reinforcement learning algorithms offer a natural, sample-based extension of dynamic programming, extending tractability to problems with high-dimensional states, continuous actions, and strategic interactions. I review the theory connecting classical planning to modern learning algorithms and demonstrate their mechanics through simulated examples in pricing, inventory control, strategic games, and preference elicitation. I also examine the practical vulnerabilities of these algorithms, noting their brittleness, sample inefficiency, sensitivity to hyperparameters, and the absence of global convergence guarantees outside of tabular settings. The successes of reinforcement learning remain strictly bounded by these constraints, as well as a reliance on accurate simulators. When guided by economic structure, reinforcement learning provides a remarkably flexible framework. It stands as an imperfect, but promising, addition to the computational economist's toolkit. A companion survey (Rust and Rawat, 2026b) covers the inverse problem of inferring preferences from observed behavior. All simulation code is publicly available.

==> appA_preliminaries/sims/robbins_monro.tex <==
\begin{table}[h]
\centering
\caption{Robbins-Monro stochastic approximation for the root of $x = \gamma x + b$ ($x^\star = 2$) with i.i.d. observation noise. A schedule converges to $x^\star$ only when $\sum_t \alpha_t = \infty$ and $\sum_t \alpha_t^2 < \infty$ both hold. Final RMS error over 100 seeds after 5000 steps.}
\label{tab:prelim_robbins_monro}
\begin{tabular}{lccc}
\hline
$\alpha_t$ & $\sum \alpha_t = \infty$ & $\sum \alpha_t^2 < \infty$ & Final RMS error \\
\hline
$1/t$ & yes & yes & 0.0451 \\
$1/t^{0.6}$ & yes & yes & 0.0766 \\
constant $0.1$ & yes & no & 0.3488 \\
$1/t^{2}$ & no & yes & 1.0827 \\
\hline
\end{tabular}
\end{table}


==> ch04_control_problems/tex/applications.tex <==
% Retired applications chapter.
%
% The canonical deployment synthesis now lives in:
%   ch13_field_deployments/tex/field_deployments.tex
%
% Build wrappers no longer include this file. Keep this pointer so old paths
% fail softly during local navigation instead of preserving a duplicate chapter.


==> ch09_rlhf/sims/job_search_horizon.tex <==
\begin{tabular}{rrrrr}
\hline
$L$ & NN RLHF $V^\pi(s_0)$ & \% of DP & DPO $V^\pi(s_0)$ & \% of DP \\
\hline
$1$ & $56.62 \pm 2.28$ & $76.4$ & $49.66 \pm 0.25$ & $67.0$ \\
$3$ & $73.89 \pm 0.04$ & $99.7$ & $69.31 \pm 0.11$ & $93.5$ \\
$5$ & $74.01 \pm 0.02$ & $99.8$ & $70.04 \pm 0.09$ & $94.5$ \\
$10$ & $74.02 \pm 0.03$ & $99.9$ & $70.29 \pm 0.08$ & $94.8$ \\
$15$ & $74.05 \pm 0.02$ & $99.9$ & $70.57 \pm 0.07$ & $95.2$ \\
$30$ & $74.05 \pm 0.02$ & $99.9$ & $70.53 \pm 0.13$ & $95.1$ \\
\hline
\end{tabular}


==> ch09_rlhf/sims/job_search_results.tex <==
\begin{tabular}{llrr}
\hline
Method & $K$ & $V^\pi(s_0)$ & \% of DP \\
\hline
DP Oracle & --- & $74.13$ & $100.0$ \\
Q-Learning & --- & $73.60 \pm 0.05$ & $99.3$ \\
\hline
NN RLHF & $25$ & $73.05 \pm 0.13$ & $98.5$ \\
DPO & $25$ & $66.39 \pm 0.34$ & $89.6$ \\
Correct & $25$ & $74.03 \pm 0.03$ & $99.9$ \\
Misspecified & $25$ & $67.34 \pm 0.38$ & $90.8$ \\
\hline
NN RLHF & $50$ & $73.31 \pm 0.08$ & $98.9$ \\
DPO & $50$ & $68.02 \pm 0.23$ & $91.8$ \\
Correct & $50$ & $74.07 \pm 0.02$ & $99.9$ \\
Misspecified & $50$ & $67.12 \pm 0.33$ & $90.6$ \\
\hline
NN RLHF & $100$ & $73.60 \pm 0.06$ & $99.3$ \\
DPO & $100$ & $69.25 \pm 0.18$ & $93.4$ \\
Correct & $100$ & $74.10 \pm 0.01$ & $100.0$ \\
Misspecified & $100$ & $67.24 \pm 0.28$ & $90.7$ \\
\hline
NN RLHF & $200$ & $73.85 \pm 0.05$ & $99.6$ \\
DPO & $200$ & $70.16 \pm 0.16$ & $94.6$ \\
Correct & $200$ & $74.12 \pm 0.00$ & $100.0$ \\
Misspecified & $200$ & $67.54 \pm 0.17$ & $91.1$ \\
\hline
NN RLHF & $500$ & $73.99 \pm 0.02$ & $99.8$ \\
DPO & $500$ & $70.60 \pm 0.10$ & $95.2$ \\
Correct & $500$ & $74.13 \pm 0.00$ & $100.0$ \\
Misspecified & $500$ & $67.55 \pm 0.15$ & $91.1$ \\
\hline
NN RLHF & $1000$ & $73.95 \pm 0.03$ & $99.8$ \\
DPO & $1000$ & $70.59 \pm 0.09$ & $95.2$ \\
Correct & $1000$ & $74.12 \pm 0.00$ & $100.0$ \\
Misspecified & $1000$ & $67.52 \pm 0.12$ & $91.1$ \\
\hline
NN RLHF & $2000$ & $74.04 \pm 0.02$ & $99.9$ \\
DPO & $2000$ & $70.41 \pm 0.07$ & $95.0$ \\
Correct & $2000$ & $74.13 \pm 0.00$ & $100.0$ \\
Misspecified & $2000$ & $67.41 \pm 0.11$ & $90.9$ \\
\hline
NN RLHF & $5000$ & $74.09 \pm 0.01$ & $99.9$ \\
DPO & $5000$ & $70.14 \pm 0.07$ & $94.6$ \\
Correct & $5000$ & $74.13 \pm 0.00$ & $100.0$ \\
Misspecified & $5000$ & $67.46 \pm 0.11$ & $91.0$ \\
\hline
\end{tabular}


==> ch10_causal/sims/confounded_ope_results.tex <==
\small
\begin{tabular}{ccccccccccc}
\toprule
& \multicolumn{2}{c}{Naive} & \multicolumn{2}{c}{Backdoor} & \multicolumn{2}{c}{Front-door} & \multicolumn{2}{c}{IV} & \multicolumn{2}{c}{Proximal} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
$\rho$ & Bias (SE) & RMSE & Bias (SE) & RMSE & Bias (SE) & RMSE & Bias (SE) & RMSE & Bias (SE) & RMSE \\
\midrule
0.0 & $-0.010$ ($0.005$) & $0.024$ & $-0.008$ ($0.005$) & $0.024$ & $-0.001$ ($0.005$) & $0.023$ & $-0.006$ ($0.028$) & $0.122$ & $-0.011$ ($0.006$) & $0.028$ \\
0.2 & $+0.060$ ($0.005$) & $0.064$ & $-0.007$ ($0.006$) & $0.025$ & $+0.003$ ($0.006$) & $0.025$ & $+0.012$ ($0.028$) & $0.125$ & $-0.012$ ($0.006$) & $0.027$ \\
0.4 & $+0.127$ ($0.005$) & $0.129$ & $-0.008$ ($0.006$) & $0.026$ & $+0.001$ ($0.006$) & $0.027$ & $+0.011$ ($0.029$) & $0.127$ & $-0.015$ ($0.006$) & $0.028$ \\
0.6 & $+0.194$ ($0.005$) & $0.195$ & $-0.007$ ($0.006$) & $0.028$ & $+0.001$ ($0.006$) & $0.028$ & $+0.020$ ($0.030$) & $0.131$ & $-0.014$ ($0.007$) & $0.033$ \\
0.8 & $+0.258$ ($0.005$) & $0.259$ & $-0.007$ ($0.006$) & $0.029$ & $-0.004$ ($0.007$) & $0.030$ & $+0.032$ ($0.030$) & $0.136$ & $-0.015$ ($0.007$) & $0.034$ \\
1.0 & $+0.321$ ($0.005$) & $0.322$ & $-0.005$ ($0.006$) & $0.028$ & $-0.004$ ($0.007$) & $0.030$ & $+0.055$ ($0.025$) & $0.123$ & $-0.015$ ($0.008$) & $0.037$ \\
\bottomrule
\end{tabular}

